Graphical posterior predictive classifier: Bayesian model averaging with particle Gibbs

In this study, we present a multi-class graphical Bayesian predictive classifier that incorporates the uncertainty in the model selection into the standard Bayesian formalism. For each class, the dependence structure underlying the observed features is represented by a set of decomposable Gaussian graphical models. Emphasis is then placed on the Bayesian model averaging which takes full account of the class-specific model uncertainty by averaging over the posterior graph model probabilities. An explicit evaluation of the model probabilities is well known to be infeasible. To address this issue, we consider the particle Gibbs strategy of Olsson et al. (2018b) for posterior sampling from decomposable graphical models which utilizes the Christmas tree algorithm of Olsson et al. (2018a) as proposal kernel. We also derive a strong hyper Markov law which we call the hyper normal Wishart law that allow to perform the resultant Bayesian calculations locally. The proposed predictive graphical classifier reveals superior performance compared to the ordinary Bayesian predictive rule that does not account for the model uncertainty, as well as to a number of out-of-the-box classifiers.

==> predictive_classification.tex <==
% -*- root: main.tex -*-


Each test sample $\testdatapnt[i]$ is by the preceding a p-dimensional column vector $\testdatapnt[i] = (x_{i1},\dots,x_{ip})'$, and correspondingly for each training sample $i \in \trdataindset$ we have $\trdatapnt[i] = (z_{i1} , \dots, z_{ip} )$.
For given classifications $\testdataindpartition, \trdataindpartition$ , each data vector assigned to a particular class $\class$ is assumed to be generated by a class-specific multivariate Gaussian distribution with mean vector $\meanvec[\class] \in \mathbb R^p$ as a class centroid, and positive definite covariance matrix $\covmat_\class \in \mathbb R^{p\times p}$. The probability density of an observed sample $\testdatapnt[i]$ (equivalently for $\trdatapnt[i]$) can then be defined as
􏰟􏰠\begin{align}
p(\testdatapnt[i] |\meanvec[\class],\covmat_\class)= (2\pi)^{-p/2} |\covmat_c|^{-1/2}  \exp \{-\frac{1}{2}(\testdatapnt[i]-\meanvec[\class])'\covmat_\class^{-1}(\testdatapnt[i]-\meanvec[\class]) \}
    \label{eq:normdensity}
\end{align}
We regard $\{\testdatapnt[i],i \in \testdataindsubset[\class]\}$ as conditionally independent outcomes of a random variable $\testdatapntrv = (\testdatapntrv[1],\dots,\testdatapntrv[p])'$ and express \ref{eq:normdensity} with $\testdatapntrv \in N(\meanvec[\class],\covmat_\class)$.


By specifying the priors of the class parameters as a product of conjugate Gaussian-Inverse-Wishart distributions, the predictive distributions can be found explicitly. The joint prior distribution of $\meanvec[\class],\covmat_\class$ is then expressed as
\begin{align}
p(\meanvec[\class],\covmat_\class)= p(\meanvec[\class]|\niwnloc[\class], \niwnscalefactor^{-1}\covmat_\class)p(\covmat_\class|\niwiwdf, \niwiwloc),
\end{align}

where $p(\meanvec[\class]|\niwnloc[\class], \niwnscalefactor^{-1}\covmat_\class)$ is the appropriate density with the hyper parameters $\niwnloc[\class] \in \mathbb R^p, \niwnscalefactor \in \mathbb R^+$, and $p(\covmat_\class|\niwiwdf, \niwiwloc)$ is the density of inverse Wishart distribution (see [8]) with the hyper parameters $\niwiwdf \in \mathbb R^+,\niwiwloc \in \mathbb R^{p\times p}$, where $\niwiwloc$ is assumed to be positive definite. The density of inverse Wishart distribution can be written as
\begin{align}
p(\covmat_\class|\niwiwdf, \niwiwloc) = (2^{\niwiwdf p/2}\Gamma_p(\niwiwdf/2))^{-1}|\niwiwloc|^{-\niwiwdf/2}|\covmat_\class|^{-(\niwiwdf+p+1)/2} \exp \{-\frac{1}{2} tr(\niwiwloc^{-1}\covmat_\class^{-1}) \} ,
\end{align}
where $\Gamma_p(\cdot)$ is the multivariate gamma function [1].
Hyper parameters $\niwnscalefactor, \niwiwdf$ and $\niwiwloc$ of the prior are the same for all classes for
any $\testdataindpartition, \trdataindpartition$ and are thus not indexed with respect to the class $\class$.
Let the sample centroid and unscaled sample covariance for class $\testdataindsubset[\class]$ be
written as
\begin{align}
    \testdatameanest[\class] =  \frac{1}{\testdatasize_\class} \sum_{i \in \testdataindsubset[\class]} \testdatapnt[i], \covmatest[{\testdataindsubset[\class]}] = \sum_{i \in \testdataindsubset[\class]} (\testdatapnt[i] - \testdatameanest[\class] )(\testdatapnt[i] - \testdatameanest[\class] )'
\end{align}
respectively, where $\testdatasize_\class = |\testdataindsubset[\class]|$.
In supervised classification, derivation of the posterior predictive distribution of test data given both training information $(\trdataset[\trdataindset],\trdataindpartition)$ and the classification $\testdataindpartition$ can be made in the following way: the training data is first used to update the prior hyper parameters  $\niwnloc[\class], \niwnscalefactor, \niwiwdf$ and $\niwiwloc$ whereafter the posterior predictive distribution is calculated by integrating out parameters with respect to the updated prior. This corresponds to
\begin{align}
    p(\testdataset[\testdataindset]|\trdataset[\trdataindset], \testdataindpartition, \trdataindpartition) =  \prod_{\class=1}^\nclasses \int_{\mathbb R^{p\times p}} \int_{\mathbb R^{p}}p(\testdataset[{\testdataindsubset[\class]}] | \meanvec[\class],\covmat_\class)p(\meanvec[\class],\covmat_\class | \trdataset[{\trdataindsubset[\class]}] , \trdataindpartition)d\meanvec[\class]d\covmat_\class
\end{align}
(5) where the above notation is simplified by omitting the hyper parameters from $p(\testdataset[\testdataindset]| \testdataindpartition, \trdataindpartition)$ [4] and
\begin{align}
p(\meanvec[\class],\covmat_\class | \trdataset[{\trdataindsubset[\class]}] , \trdataindpartition) = \frac{p(\trdataset[{\trdataindsubset[\class]}] | \meanvec[\class],\covmat_\class)p(\meanvec[\class],\covmat_\class)}{\int_{\mathbb R^{p\times p}} \int_{\mathbb R^{p}}p(\trdataset[{\trdataindsubset[\class]}] | \meanvec[\class],\covmat_\class)p(\meanvec[\class],\covmat_\class)d\meanvec[\class]d\covmat_\class}
\end{align}
is the posterior distribution of $\meanvec[\class],\covmat_\class$ based on the prior $p(\meanvec[\class],\covmat_\class)$ in (2) and the data $\trdataset[{\trdataindsubset[\class]}]$ in class $\class$ of $\trdataindpartition$.
